Identification Under the Semantic Effective Secrecy Constraint

The problem of identification over a discrete memoryless wiretap channel is examined under the criterion of semantic effective secrecy. This secrecy criterion guarantees both the requirement of semantic secrecy and of stealthy communication. Additionally, we introduce the related problem of combining approximation-of-output statistics and transmission. We derive a capacity theorem for approximation-of-output statistics transmission codes. For a general model, we present lower and upper bounds on the capacity, showing that these bounds are tight for more capable wiretap channels. We also provide illustrative examples for more capable wiretap channels, along with examples of wiretap channel classes where a gap exists between the lower and upper bounds.

==> local-shorthands.tex <==
% project specific shorthands go here

% for latexdiff: marks parts which should not
% be analyzed by latexdiff
\newenvironment{DIFnomarkup}{}{} 

\NewDocumentCommand{\defname}{om}{\emph{#2}\IfValueT{#1}{~(#1)}}

\newcommand{\code}{\cC}

\DeclareMathOperator{\ESinfOp}{ES}
\newcommand{\ESinf}[4]{\ESinfOp_{#1}({#2} \to {#3}, {#4})}
\DeclareMathOperator{\BEC}{BEC}
\DeclareMathOperator{\BSC}{BSC}
% \DeclareMathOperator{\supp}{supp}

\newcommand{\capacity}{\mathsf{C}}

\ExplSyntaxOn
  \clist_map_inline:nn {T,EST,ID,ESID,DI,SID,ST,AOST} {
    \cs_new_nopar:cpn { cap #1 } {\capacity\sb{\mathsf{#1}}}
  }
  \clist_map_inline:nn {aost,aos,esid,st,est} {
    \cs_new_nopar:cpn { P #1 } {\cP\sb{\mathsf{\MakeUppercase{#1}}}}
  }
\ExplSyntaxOff


\ifdraft
  \let \fxcolor \color
  \let \fxtextcolor \textcolor
\else
  \NewExpandableDocumentCommand \fxcolor {m} {}
  \NewExpandableDocumentCommand \fxtextcolor {m} {}
\fi
\ExplSyntaxOn
\makeatletter
\NewExpandableDocumentCommand \fxchecked {O{}m} {
  \fxtextcolor{green}{~(checked \@fxsignature{#1:}~{#2})}
}
\clist_map_inline:nn {ai,jr,bb,cd,rf,up} {
  \cs_new_nopar:cpn { #1 checked } { \fxchecked[\MakeUppercase{#1}] }
}
\makeatother
\ExplSyntaxOff

%BB's todo command, comment out and check compilation before submission
\ifdraft % like commenting out if document is compiled with option 'final'
  \newcommand{\todo}[1]{{\color{red}{\textbf{Todo: \emph{#1}}}}}
\fi

% vim: ts=2 sw=2

